Leveraging AES Padding: dBs for Nothing and FEC for Free in IoT Systems

The Internet of Things (IoT) represents a significant advancement in digital technology, with its rapidly growing network of interconnected devices. This expansion, however, brings forth critical challenges in data security and reliability, especially under the threat of increasing cyber vulnerabilities. Addressing the security concerns, the Advanced Encryption Standard (AES) is commonly employed for secure encryption in IoT systems. Our study explores an innovative use of AES, by repurposing AES padding bits for error correction and thus introducing a dual-functional method that seamlessly integrates error-correcting capabilities into the standard encryption process. The integration of the state-of-the-art Guessing Random Additive Noise Decoder (GRAND) in the receiver's architecture facilitates the joint decoding and decryption process. This strategic approach not only preserves the existing structure of the transmitter but also significantly enhances communication reliability in noisy environments, achieving a notable over 3 dB gain in Block Error Rate (BLER). Remarkably, this enhanced performance comes with a minimal power overhead at the receiver - less than 15% compared to the traditional decryption-only process, underscoring the efficiency of our hardware design for IoT applications. This paper discusses a comprehensive analysis of our approach, particularly in energy efficiency and system performance, presenting a novel and practical solution for reliable IoT communications.

==> 5_system_analysis_backup.tex <==


\section{System Analysis} \label{sec:system_analysis}

This section presents the results of evaluating the performance of AES as an error-correcting code in comparison to different transmitter setups discussed in Section~\ref{sec:proposed_system}. We also include hardware simulation results for the receiver architecture, focusing on power, throughput, energy per bit, and area. The receiver system was designed and implemented using 28nm CMOS technology, and the results were obtained from post-synthesis simulations at 0.9V and 100MHz.



\subsection{Error Correcting Capability}
In our error-correcting performance evaluation, binary messages of length k-bits, chosen uniformly from $F^{k}_{2}$, were transmitted using Binary Phase Shift Keying (BPSK) over an Additive White Gaussian Noise (AWGN) channel. We maintained an equal number of redundancy bits across different transmitter encoding scenarios. This approach was essential since the error-correcting performance of the GRAND decoder is influenced by the number of redundancy bits~\cite{Duffy_2019}. Performance metrics such BER and BLER were analyzed based on the energy per information bit to noise power spectral density ratio ($Eb/N_{0}$).

In our simulations, we investigated three distinct scenarios:
\begin{itemize}
    \item \textbf{Baseline Encryption-Only without Encoding:} This system focuses solely on encryption, applying hard decoding where any bit error leads to decoding failure. It is a straightforward approach emphasizing data security, without incorporating any additional encoding.
    \item \textbf{Separate Encryption and Encoding:} This setup uses ORBGRAND for decoding, leveraging soft information from signal reliability. It combines encryption with subsequent encoding, enhancing error correction while maintaining secure data transmission. The choice of ORBGRAND is due to its superior error-correcting capabilities, flexibility, and energy efficiency in hardware, making it a suitable option for this architecture~\cite{10067519}.
    \item \textbf{Proposed AES as Error Correction:} This method innovatively combines joint decoding and decryption using ORBGRAND. \textcolor{blue}{It enhances error correction capabilities within the framework of AES encryption, providing a balanced approach to secure and reliable data transmission.}
\end{itemize}


%Figure~\ref{fig:(128,116)_results},~\ref{fig:(128,120)_results} and~\ref{fig:(128,124)_results} provide a comprehensive analysis of BER and BLER against $Eb/N_{0}$. These figures represent different code rates of 0.91, 0.94, and 0.97, offering a detailed comparison of the error-correcting performance of the AES error correction scheme under various conditions and scenarios. The proposed AES error correction scheme showcased a remarkable improvement over the encryption-only system, particularly in code rate scenarios of $R=0.91$. This was evident in a significant 3dB gain in the BER under $10^{-5}$, signifying a substantial enhancement in system reliability without any modifications to the transmitter's setup. Particularly, the first set of trails with code rate 0.91 further included multiple coding schemes such as RLC and CA-POLAR as the encoding approach, to compare the error correction capabilities of our approach. It is evident that our approach performs as good as an RLC coding scheme in low $Eb/N_{0}$s with slight decline in higher $Eb/N_{0}$. However, we consistently outperform not only the ``no encoding" scenario but also the ``CA-POLAR" code which is very commonly used in practical applications. This shows that the AES as error correction is in fact a good error correction scheme that comes at no cost with the encryption.


% \begin{figure*}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/(128,116).pdf}
%     \caption{BER (left) and BLER (right) vs. $Eb/N_{0}$ for redundancy bits = 12-bit}
%     \label{fig:(128,116)_results}
% \end{figure*}

% \begin{figure*}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/(128,120).pdf}
%     \caption{BER (left) and BLER (right) vs. $Eb/N_{0}$ for redundancy bits = 8-bit}
%     \label{fig:(128,120)_results}
% \end{figure*}

%% Comparison
\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figures/(128,116)_phrase.pdf}
    \caption{BER (left) and BLER (right) vs. $Eb/N_{0}$ for padding bits = 12-bit}
    \label{fig:(128,116)_results}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figures/(128,120)_phrase.pdf}
    \caption{BER (left) and BLER (right) vs. $Eb/N_{0}$ for padding bits = 8-bit}
    \label{fig:(128,120)_results}
\end{figure*}

% \begin{figure*}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/(128,124).pdf}
%     \caption{BER (left) and BLER (right) vs. $Eb/N_{0}$ for redundancy bits = 4-bit}
%     \label{fig:(128,124)_results}
% \end{figure*}


Figures~\ref{fig:(128,116)_results} and~\ref{fig:(128,120)_results} provide a comprehensive analysis of BER and BLER against $Eb/N{0}$. These figures showcase different scenarios with padding bits of 8-bit and 12-bit. The proposed AES error correction scheme significantly improves over the baseline encryption-only system, especially with 12-bit padding. This improvement is particularly remarkable in the BER under $10^{-4}$, indicating a substantial improvement in the reliability of the system.


The first set of trials with 12-bit padding demonstrated the robustness of our AES error correction strategy. It was compared with state-of-the-art encoding and decoding schemes such as RLC~\cite{article} and CA-Polar~\cite{7055304} for encoding, and ORBGRAND~\cite{9872126} and CRC-Aided Successive Cancellation List (CA-SCL)~\cite{6297420} for decoding. Our approach not only outperformed the ``no encoding" scenario but also showed competitive capabilities against the widely used "CA-POLAR" code with CA-SCL decoding. Significantly, this level of error correction effectiveness was achieved with less than 10\% of the redundancy bits, underscoring the efficiency of our method. Additionally, it is noteworthy that ORBGRAND displayed significantly superior performance over the state-of-the-art CA-SCL decoder in both BER and BLER metrics, further establishing its effectiveness.


In scenarios involving 8-bit and 12-bit redundancy, our proposed system consistently outperformed the baseline encryption-only setup, demonstrating its versatility across different conditions. When compared with systems employing separate encryption and encoding — where encryption is followed by encoding — our integrated approach maintained similar levels of BER and BLER. This performance comparability, despite different operational methodologies, highlights the effectiveness of our proposed method in enhancing communication reliability without altering the security level. Our approach maintains the same security standards while significantly improving reliability, demonstrating a balanced advancement in secure and reliable IoT communications.

% However, it was noted that in higher $Eb/N_{0}$ scenarios, which represent low noise conditions, our system experienced a slight performance decrease relative to the encrypt-and-encode system. (REASONING REQUIRED)
In high $Eb/N_{0}$ scenarios, which typically indicate low noise conditions, our AES-based error correction system demonstrated a slight decline in performance relative to the separate encrypt-and-encode system. This can be attributed to the inherent nature of AES's non-linear codebook. Unlike linear codes, where the minimum Hamming distance is consistent across all codewords, the AES codebook does not maintain this uniformity~\cite{wei1991generalized}. At higher $Eb/N_{0}$ levels, noise is more likely to cause single-bit errors. For linear codes, this generally results in significant Hamming distances to the nearest codeword, maintaining error correction effectiveness. However, in the AES system, due to its non-linear codebook, a single-bit error for certain codewords may result in an erroneous codeword being closer, leading to decreased error correction performance. This characteristic becomes more pronounced at higher $Eb/N_{0}$, hence the observed degradation in our system's performance.

Despite this minor decline in high $Eb/N_{0}$ conditions, our proposed system consistently outperformed the encryption-only approach in terms of lower BER and BLER. Achieving a BER better than $10^{-4}$ is particularly significant in IEEE 802.15.4 standard~\cite{6749420,alnuaimi2006performance}, underscoring the practicality and applicability of our system in real-world settings. This finding highlights the potential of our proposed AES error correction scheme in enhancing the reliability of communication systems, particularly in IoT environments where efficient and secure data transmission is crucial.

% \begin{figure*}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/(128,116).pdf}
%     \caption{BER (left) and BLER (right) vs. $Eb/N_{0}$ for code rate R = 0.91}
%     \label{fig:(128,116)_results}
% \end{figure*}

\subsection{Hardware Analysis}
%\input{table_no_area}
%\input{table_with_latency}
\input{tables/table_with_all_no_op}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/area.pdf}
    \caption{Area comparison in different receiver architectures. Proposed(left), separate with 8-bit padding(middle) and separate with 12-it padding(right)}
    \label{fig:area}
\end{figure}

The hardware analysis in our study compares the performance of three different receiver architectures: our proposed system with integrated joint ORBGRAND and AES decoding and decryption, a baseline system focusing only on AES decryption without error correction, and a separate system that combines ORBGRAND decoding with subsequent AES decryption. This comprehensive analysis, detailed in Table~\ref{tab:hardware_results}, examines power consumption, latency, goodput, and energy efficiency under various $Eb/N_{0}$ scenarios along with different numbers of padding bits. The findings provide valuable insight into the operational efficiencies and energy demands of these systems, providing a clear understanding of their relative performances in different signal-to-noise ratio environments.

The baseline system, solely relying on AES decryption, displays consistent power consumption and latency across all noise levels, maintaining uniform operation regardless of channel conditions. However, its goodput and energy per bit, tied to the actual payload data ($k$-bit), are influenced by the size of the padding bits, thus varying with the number of redundancy bits used. This variation in goodput and energy efficiency reflects the baseline's dependence on payload size in different operational scenarios.

In contrast, our proposed receiver system experiences an additional power overhead from the error pattern generator. Remarkably, in high $Eb/N_{0}$ scenarios, this overhead is less than 15\% compared to the baseline decryption-only system, a rate that remains fairly consistent even in lower $Eb/N_{0}$ scenarios. The separate system, which employs sequential ORBGRAND decoding and AES decryption, demonstrates lower power consumption in lower $Eb/N_{0}$ scenarios. This is attributed to the system's operational strategy, where it runs the error pattern generator and syndrome check until successful decoding, followed by a single instance of AES decryption.

In the context of latency, our proposed system demonstrates no degradation compared to the baseline system in high $Eb/N_{0}$ scenarios, maintaining a consistent latency of 130ns for the entire decoding and decryption process, which is a direct result of the pipelined and parallel processing design. This performance is notably superior to the separate decoding and decryption system, which requires 150ns for the same process. The enhanced latency of our system translates into higher goodput, making it highly advantageous for IoT receiver applications where efficiency is key. However, in lower $Eb/N_{0}$ conditions, the need for frequent generation of new error patterns and padding checks in our system results in increased latency, which adversely impacts the goodput. This trade-off highlights the balance our system strikes between latency and error correction, adapting its performance according to varying channel conditions.

In the high $Eb/N_{0}$ scenarios, the energy per bit metric for our proposed system demonstrates an overhead of less than 15\% compared to the baseline system. Despite the higher power demand of the proposed system, its superior goodput efficiency effectively compensates for this, resulting in a comparably efficient energy per bit performance. Furthermore, when we compare the proposed system with the separate system, the energy per bit figures are comparable across the two architectures, particularly notable in high $Eb/N_{0}$ conditions. In contrast, in low $Eb/N_{0}$ scenarios, despite having similar power consumption levels, the proposed system's reduced goodput leads to a relative increase in energy per bit, highlighting the impact of operational efficiency on energy metrics in different noise environments.

The area comparison between our proposed receiver architecture and the separate systems is illustrated in Figure~\ref{fig:area}. In our design, both the AES and error pattern generator components are optimized for low latency, tailored to a 128-bit block size. This approach ensures a consistent AES area across different systems. The area of the error pattern generator varies with the codeword length ($n$), but its basic architecture is designed to minimize latency in error pattern generation for all systems. Consequently, our proposed receiver architecture, while maintaining a similar AES area, benefits from a more compact error pattern generator due to the shorter codeword length, enhancing efficiency in space-constrained IoT applications.

The area efficiency of our proposed receiver system is enhanced due to the absence of a large $H$-matrix for syndrome check, a feature required in the separate systems. In the separate decoding and decryption system, the area for syndrome check is directly proportional to the product of the number of redundancy bits ($n-k$) and the codeword length ($n$), necessitating substantial storage in registers. Our system's approach, which involves padding check instead of syndrome check, eliminates the need for this extensive matrix storage. This design choice not only reduces the area by approximately 28\% compared to the separate systems but also becomes more beneficial at lower code rates. The absence of additional area requirements for padding check in our architecture emphasizes its suitability for IoT applications, where space and resource constraints are critical factors.

The overhead of area in our proposed system is mainly due to the error pattern generator, which is 50.2kGE (kilo-Gate Equivalent). However, this is still smaller than the separate system, which requires over 67kGE for error-correcting capabilities compared to a baseline receiver. This highlights the balance our system strikes between maintaining error-correcting capabilities and efficient use of space, vital in energy and area-constrained IoT environments.


==> tables/table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{2}
\begin{threeparttable}
\centering    
\caption{\centering Performance comparison in different with different numbers of splits}
\label{tab:hardware_results}

\begin{tabular}
{|c|cccccccccccccccccccccc|}
\hline
\multirow{4}{*}{Eb/N0} & \multicolumn{6}{c|}{Power   (mW)} & \multicolumn{6}{c|}{Goodput   (Mbps)} & \multicolumn{6}{c|}{Energy/bit   (pJ/bit)} & \multicolumn{4}{c|}{Area   (GE)} \\ \cline{2-23} 
 & \multicolumn{22}{c|}{Code   rate (R)} \\ \cline{2-23} 
 & \multicolumn{2}{c|}{0.97} & \multicolumn{2}{c|}{0.94} & \multicolumn{2}{c|}{0.91} & \multicolumn{2}{c|}{0.97} & \multicolumn{2}{c|}{0.94} & \multicolumn{2}{c|}{0.91} & \multicolumn{2}{c|}{0.97} & \multicolumn{2}{c|}{0.94} & \multicolumn{2}{c|}{0.91} & \multicolumn{1}{c|}{*} & \multicolumn{1}{c|}{0.97} & \multicolumn{1}{c|}{0.94} & 0.91 \\ \cline{2-23} 
 & \multicolumn{1}{c|}{B\tnote{a}}  & \multicolumn{1}{c|}{P\tnote{b}}  & \multicolumn{1}{c|}{B\tnote{a}}  & \multicolumn{1}{c|}{P\tnote{b}}  & \multicolumn{1}{c|}{B\tnote{a}}  & \multicolumn{1}{c|}{P\tnote{b}}  & \multicolumn{1}{c|}{B\tnote{a}}  & \multicolumn{1}{c|}{P\tnote{b}}  & \multicolumn{1}{c|}{B\tnote{a}}  & \multicolumn{1}{c|}{P\tnote{b}}  & \multicolumn{1}{c|}{B\tnote{a}}  & \multicolumn{1}{c|}{P\tnote{b}}  & \multicolumn{1}{c|}{B\tnote{a}}  & \multicolumn{1}{c|}{P\tnote{b}}  & \multicolumn{1}{c|}{B\tnote{a}}  & \multicolumn{1}{c|}{P\tnote{b}}  & \multicolumn{1}{c|}{B\tnote{a}}  & \multicolumn{1}{c|}{P\tnote{b}}  & \multicolumn{1}{c|}{B\tnote{a}}  & \multicolumn{3}{c|}{P\tnote{b}}  \\ \hline
5 & \multicolumn{1}{c|}{1.46} & \multicolumn{1}{c|}{1.05} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{0.69} & \multicolumn{1}{c|}{1.35} & \multicolumn{1}{c|}{0.4} & \multicolumn{1}{c|}{238} & \multicolumn{1}{c|}{469} & \multicolumn{1}{c|}{64} & \multicolumn{1}{c|}{129} & \multicolumn{1}{c|}{17} & \multicolumn{1}{c|}{22} & \multicolumn{1}{c|}{6.14} & \multicolumn{1}{c|}{2.24} & \multicolumn{1}{c|}{21.9} & \multicolumn{1}{c|}{5.36} & \multicolumn{1}{c|}{78.8} & \multicolumn{1}{c|}{18.3} & \multicolumn{1}{c|}{\multirow{6}{*}{50K}} & \multicolumn{1}{c|}{\multirow{6}{*}{77K}} & \multicolumn{1}{c|}{\multirow{6}{*}{83K}} & \multirow{6}{*}{91K} \\ \cline{1-19}
6 & \multicolumn{1}{c|}{1.42} & \multicolumn{1}{c|}{1.15} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{1.09} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{1.01} & \multicolumn{1}{c|}{529} & \multicolumn{1}{c|}{644} & \multicolumn{1}{c|}{321} & \multicolumn{1}{c|}{443} & \multicolumn{1}{c|}{176} & \multicolumn{1}{c|}{203} & \multicolumn{1}{c|}{2.69} & \multicolumn{1}{c|}{1.79} & \multicolumn{1}{c|}{4.37} & \multicolumn{1}{c|}{2.47} & \multicolumn{1}{c|}{7.93} & \multicolumn{1}{c|}{5} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\ \cline{1-19}
7 & \multicolumn{1}{c|}{1.39} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.39} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{812} & \multicolumn{1}{c|}{758} & \multicolumn{1}{c|}{726} & \multicolumn{1}{c|}{690} & \multicolumn{1}{c|}{627} & \multicolumn{1}{c|}{596} & \multicolumn{1}{c|}{1.71} & \multicolumn{1}{c|}{1.58} & \multicolumn{1}{c|}{1.92} & \multicolumn{1}{c|}{1.72} & \multicolumn{1}{c|}{2.23} & \multicolumn{1}{c|}{1.99} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\ \cline{1-19}
8 & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{919} & \multicolumn{1}{c|}{808} & \multicolumn{1}{c|}{878} & \multicolumn{1}{c|}{771} & \multicolumn{1}{c|}{832} & \multicolumn{1}{c|}{728} & \multicolumn{1}{c|}{1.5} & \multicolumn{1}{c|}{1.48} & \multicolumn{1}{c|}{1.57} & \multicolumn{1}{c|}{1.54} & \multicolumn{1}{c|}{1.66} & \multicolumn{1}{c|}{1.65} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\ \cline{1-19}
9 & \multicolumn{1}{c|}{1.37} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{947} & \multicolumn{1}{c|}{823} & \multicolumn{1}{c|}{915} & \multicolumn{1}{c|}{794} & \multicolumn{1}{c|}{882} & \multicolumn{1}{c|}{763} & \multicolumn{1}{c|}{1.45} & \multicolumn{1}{c|}{1.46} & \multicolumn{1}{c|}{1.51} & \multicolumn{1}{c|}{1.5} & \multicolumn{1}{c|}{1.56} & \multicolumn{1}{c|}{1.57} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\ \cline{1-19}
10 & \multicolumn{1}{c|}{1.37} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{953} & \multicolumn{1}{c|}{826} & \multicolumn{1}{c|}{922} & \multicolumn{1}{c|}{799} & \multicolumn{1}{c|}{891} & \multicolumn{1}{c|}{772} & \multicolumn{1}{c|}{1.44} & \multicolumn{1}{c|}{1.45} & \multicolumn{1}{c|}{1.49} & \multicolumn{1}{c|}{1.49} & \multicolumn{1}{c|}{1.54} & \multicolumn{1}{c|}{1.55} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\ \hline

\end{tabular}

     \begin{tablenotes} \footnotesize
       \item [a] Baseline receiver system, ORBGRAND decoding followed by AES decryption
       \item [b] Proposed receiver system, joint decoding and decryption
     \end{tablenotes}
  \end{threeparttable}
     }
\end{table*}



==> tables/table_no_area.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}

% \begin{table*}[]
% \resizebox{\textwidth}{!}{%
% \renewcommand{\arraystretch}{2}
% \begin{threeparttable}
% \centering    
% \caption{\centering Performance comparison in different with different numbers of splits}
% \label{tab:hardware_results}

% \begin{tabular}{|c|cccccccccccccccccc|}
% \hline
% \multirow{4}{*}{\textbf{EbN0}} & \multicolumn{6}{c|}{\textbf{Power   (mW)}} & \multicolumn{6}{c|}{\textbf{Goodput   (Mbps)}} & \multicolumn{6}{c|}{\textbf{Energy/bit   (pJ/bit)}} \\ \cline{2-19} 
%  & \multicolumn{18}{c|}{\textbf{Code   rate (R)}} \\ \cline{2-19} 
%  & \multicolumn{2}{c|}{\textbf{0.97}} & \multicolumn{2}{c|}{\textbf{0.94}} & \multicolumn{2}{c|}{\textbf{0.91}} & \multicolumn{2}{c|}{\textbf{0.97}} & \multicolumn{2}{c|}{\textbf{0.94}} & \multicolumn{2}{c|}{\textbf{0.91}} & \multicolumn{2}{c|}{\textbf{0.97}} & \multicolumn{2}{c|}{\textbf{0.94}} & \multicolumn{2}{c|}{\textbf{0.91}} \\ \cline{2-19} 
%  & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \textbf{P} \\ \hline\hline
% 5 & \multicolumn{1}{c|}{1.05} & \multicolumn{1}{c|}{1.46} & \multicolumn{1}{c|}{0.69} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{0.4} & \multicolumn{1}{c|}{1.35} & \multicolumn{1}{c|}{469} & \multicolumn{1}{c|}{238} & \multicolumn{1}{c|}{129} & \multicolumn{1}{c|}{64} & \multicolumn{1}{c|}{22} & \multicolumn{1}{c|}{17} & \multicolumn{1}{c|}{2.24} & \multicolumn{1}{c|}{6.14} & \multicolumn{1}{c|}{5.36} & \multicolumn{1}{c|}{21.9} & \multicolumn{1}{c|}{18.3} & 78.8 \\ \hline
% 6 & \multicolumn{1}{c|}{1.15} & \multicolumn{1}{c|}{1.42} & \multicolumn{1}{c|}{1.09} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{1.01} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{644} & \multicolumn{1}{c|}{529} & \multicolumn{1}{c|}{443} & \multicolumn{1}{c|}{321} & \multicolumn{1}{c|}{203} & \multicolumn{1}{c|}{176} & \multicolumn{1}{c|}{1.79} & \multicolumn{1}{c|}{2.69} & \multicolumn{1}{c|}{2.47} & \multicolumn{1}{c|}{4.37} & \multicolumn{1}{c|}{5.00} & 7.93 \\ \hline
% 7 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.39} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.39} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{758} & \multicolumn{1}{c|}{812} & \multicolumn{1}{c|}{690} & \multicolumn{1}{c|}{726} & \multicolumn{1}{c|}{596} & \multicolumn{1}{c|}{627} & \multicolumn{1}{c|}{1.58} & \multicolumn{1}{c|}{1.71} & \multicolumn{1}{c|}{1.72} & \multicolumn{1}{c|}{1.92} & \multicolumn{1}{c|}{1.99} & 2.23 \\ \hline
% 8 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{808} & \multicolumn{1}{c|}{919} & \multicolumn{1}{c|}{771} & \multicolumn{1}{c|}{878} & \multicolumn{1}{c|}{728} & \multicolumn{1}{c|}{832} & \multicolumn{1}{c|}{1.48} & \multicolumn{1}{c|}{1.5} & \multicolumn{1}{c|}{1.54} & \multicolumn{1}{c|}{1.57} & \multicolumn{1}{c|}{1.65} & 1.66 \\ \hline
% 9 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.37} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{823} & \multicolumn{1}{c|}{947} & \multicolumn{1}{c|}{794} & \multicolumn{1}{c|}{915} & \multicolumn{1}{c|}{763} & \multicolumn{1}{c|}{882} & \multicolumn{1}{c|}{1.46} & \multicolumn{1}{c|}{1.45} & \multicolumn{1}{c|}{1.5} & \multicolumn{1}{c|}{1.51} & \multicolumn{1}{c|}{1.57} & 1.56 \\ \hline
% 10 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.37} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{826} & \multicolumn{1}{c|}{953} & \multicolumn{1}{c|}{799} & \multicolumn{1}{c|}{922} & \multicolumn{1}{c|}{772} & \multicolumn{1}{c|}{891} & \multicolumn{1}{c|}{1.45} & \multicolumn{1}{c|}{1.44} & \multicolumn{1}{c|}{1.49} & \multicolumn{1}{c|}{1.49} & \multicolumn{1}{c|}{1.55} & 1.54 \\ \hline


% \end{tabular}

%      \begin{tablenotes} \footnotesize
%        \item [a] Baseline receiver system, ORBGRAND decoding followed by AES decryption
%        \item [b] Proposed receiver system, joint decoding and decryption
%      \end{tablenotes}
%   \end{threeparttable}
%      }
% \end{table*}
    
    


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{2}
\begin{threeparttable}
\centering    
\caption{\centering Performance comparison in different  receiver architecture}
\label{tab:hardware_results}

\begin{tabular}{|c||cccccccccccccccccc|}
\hline
\multirow{4}{*}{\textbf{EbN0}} & \multicolumn{18}{c|}{\textbf{Code   rate (R)}} \\ \cline{2-19} 
 & \multicolumn{2}{c|}{\textbf{0.97}} & \multicolumn{2}{c|}{\textbf{0.94}} & \multicolumn{2}{c||}{\textbf{0.91}} & \multicolumn{2}{c|}{\textbf{0.97}} & \multicolumn{2}{c|}{\textbf{0.94}} & \multicolumn{2}{c||}{\textbf{0.91}} & \multicolumn{2}{c|}{\textbf{0.97}} & \multicolumn{2}{c|}{\textbf{0.94}} & \multicolumn{2}{c|}{\textbf{0.91}} \\ \cline{2-19} 
 & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c||}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c||}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \textbf{P} \\ \cline{2-19} 
 & \multicolumn{6}{c||}{\textbf{Power   (mW)}} & \multicolumn{6}{c||}{\textbf{Goodput   (Mbps)}} & \multicolumn{6}{c|}{\textbf{Energy/bit   (pJ/bit)}} \\ \hline\hline
5 & \multicolumn{1}{c|}{1.05} & \multicolumn{1}{c|}{1.46} & \multicolumn{1}{c|}{0.69} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{0.4} & \multicolumn{1}{c||}{1.35} & \multicolumn{1}{c|}{469} & \multicolumn{1}{c|}{238} & \multicolumn{1}{c|}{129} & \multicolumn{1}{c|}{64} & \multicolumn{1}{c|}{22} & \multicolumn{1}{c||}{17} & \multicolumn{1}{c|}{2.24} & \multicolumn{1}{c|}{6.14} & \multicolumn{1}{c|}{5.36} & \multicolumn{1}{c|}{21.9} & \multicolumn{1}{c|}{18.3} & 78.8 \\ \hline
6 & \multicolumn{1}{c|}{1.15} & \multicolumn{1}{c|}{1.42} & \multicolumn{1}{c|}{1.09} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{1.01} & \multicolumn{1}{c||}{1.4} & \multicolumn{1}{c|}{644} & \multicolumn{1}{c|}{529} & \multicolumn{1}{c|}{443} & \multicolumn{1}{c|}{321} & \multicolumn{1}{c|}{203} & \multicolumn{1}{c||}{176} & \multicolumn{1}{c|}{1.79} & \multicolumn{1}{c|}{2.69} & \multicolumn{1}{c|}{2.47} & \multicolumn{1}{c|}{4.37} & \multicolumn{1}{c|}{5.00} & 7.93 \\ \hline
7 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.39} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.39} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c||}{1.4} & \multicolumn{1}{c|}{758} & \multicolumn{1}{c|}{812} & \multicolumn{1}{c|}{690} & \multicolumn{1}{c|}{726} & \multicolumn{1}{c|}{596} & \multicolumn{1}{c||}{627} & \multicolumn{1}{c|}{1.58} & \multicolumn{1}{c|}{1.71} & \multicolumn{1}{c|}{1.72} & \multicolumn{1}{c|}{1.92} & \multicolumn{1}{c|}{1.99} & 2.23 \\ \hline
8 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c||}{1.38} & \multicolumn{1}{c|}{808} & \multicolumn{1}{c|}{919} & \multicolumn{1}{c|}{771} & \multicolumn{1}{c|}{878} & \multicolumn{1}{c|}{728} & \multicolumn{1}{c||}{832} & \multicolumn{1}{c|}{1.48} & \multicolumn{1}{c|}{1.5} & \multicolumn{1}{c|}{1.54} & \multicolumn{1}{c|}{1.57} & \multicolumn{1}{c|}{1.65} & 1.66 \\ \hline
9 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.37} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c||}{1.38} & \multicolumn{1}{c|}{823} & \multicolumn{1}{c|}{947} & \multicolumn{1}{c|}{794} & \multicolumn{1}{c|}{915} & \multicolumn{1}{c|}{763} & \multicolumn{1}{c||}{882} & \multicolumn{1}{c|}{1.46} & \multicolumn{1}{c|}{1.45} & \multicolumn{1}{c|}{1.5} & \multicolumn{1}{c|}{1.51} & \multicolumn{1}{c|}{1.57} & 1.56 \\ \hline
10 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.37} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c||}{1.38} & \multicolumn{1}{c|}{826} & \multicolumn{1}{c|}{953} & \multicolumn{1}{c|}{799} & \multicolumn{1}{c|}{922} & \multicolumn{1}{c|}{772} & \multicolumn{1}{c||}{891} & \multicolumn{1}{c|}{1.45} & \multicolumn{1}{c|}{1.44} & \multicolumn{1}{c|}{1.49} & \multicolumn{1}{c|}{1.49} & \multicolumn{1}{c|}{1.55} & 1.54 \\ \hline



\end{tabular}

     \begin{tablenotes} \footnotesize
       \item B: Baseline receiver system, ORBGRAND decoding followed by AES decryption
       \item P: Proposed receiver system, joint ORBGRAND decoding and AES decryption
     \end{tablenotes}
  \end{threeparttable}
     }
\end{table*}

==> tables/table_with_all.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}

% \begin{table*}[]
% \resizebox{\textwidth}{!}{%
% \renewcommand{\arraystretch}{2}
% \begin{threeparttable}
% \centering    
% \caption{\centering Performance comparison in different with different numbers of splits}
% \label{tab:hardware_results}

% \begin{tabular}{|c|cccccccccccccccccc|}
% \hline
% \multirow{4}{*}{\textbf{EbN0}} & \multicolumn{6}{c|}{\textbf{Power   (mW)}} & \multicolumn{6}{c|}{\textbf{Goodput   (Mbps)}} & \multicolumn{6}{c|}{\textbf{Energy/bit   (pJ/bit)}} \\ \cline{2-19} 
%  & \multicolumn{18}{c|}{\textbf{Code   rate (R)}} \\ \cline{2-19} 
%  & \multicolumn{2}{c|}{\textbf{4-bit}} & \multicolumn{2}{c|}{\textbf{8-bit}} & \multicolumn{2}{c|}{\textbf{12-bit}} & \multicolumn{2}{c|}{\textbf{4-bit}} & \multicolumn{2}{c|}{\textbf{8-bit}} & \multicolumn{2}{c|}{\textbf{12-bit}} & \multicolumn{2}{c|}{\textbf{4-bit}} & \multicolumn{2}{c|}{\textbf{8-bit}} & \multicolumn{2}{c|}{\textbf{12-bit}} \\ \cline{2-19} 
%  & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \textbf{P} \\ \hline\hline
% 5 & \multicolumn{1}{c|}{1.05} & \multicolumn{1}{c|}{1.46} & \multicolumn{1}{c|}{0.69} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{0.4} & \multicolumn{1}{c|}{1.35} & \multicolumn{1}{c|}{469} & \multicolumn{1}{c|}{238} & \multicolumn{1}{c|}{129} & \multicolumn{1}{c|}{64} & \multicolumn{1}{c|}{22} & \multicolumn{1}{c|}{17} & \multicolumn{1}{c|}{2.24} & \multicolumn{1}{c|}{6.14} & \multicolumn{1}{c|}{5.36} & \multicolumn{1}{c|}{21.9} & \multicolumn{1}{c|}{18.3} & 78.8 \\ \hline
% 6 & \multicolumn{1}{c|}{1.15} & \multicolumn{1}{c|}{1.42} & \multicolumn{1}{c|}{1.09} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{1.01} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{644} & \multicolumn{1}{c|}{529} & \multicolumn{1}{c|}{443} & \multicolumn{1}{c|}{321} & \multicolumn{1}{c|}{203} & \multicolumn{1}{c|}{176} & \multicolumn{1}{c|}{1.79} & \multicolumn{1}{c|}{2.69} & \multicolumn{1}{c|}{2.47} & \multicolumn{1}{c|}{4.37} & \multicolumn{1}{c|}{5.00} & 7.93 \\ \hline
% 7 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.39} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.39} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{758} & \multicolumn{1}{c|}{812} & \multicolumn{1}{c|}{690} & \multicolumn{1}{c|}{726} & \multicolumn{1}{c|}{596} & \multicolumn{1}{c|}{627} & \multicolumn{1}{c|}{1.58} & \multicolumn{1}{c|}{1.71} & \multicolumn{1}{c|}{1.72} & \multicolumn{1}{c|}{1.92} & \multicolumn{1}{c|}{1.99} & 2.23 \\ \hline
% 8 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{808} & \multicolumn{1}{c|}{919} & \multicolumn{1}{c|}{771} & \multicolumn{1}{c|}{878} & \multicolumn{1}{c|}{728} & \multicolumn{1}{c|}{832} & \multicolumn{1}{c|}{1.48} & \multicolumn{1}{c|}{1.5} & \multicolumn{1}{c|}{1.54} & \multicolumn{1}{c|}{1.57} & \multicolumn{1}{c|}{1.65} & 1.66 \\ \hline
% 9 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.37} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{823} & \multicolumn{1}{c|}{947} & \multicolumn{1}{c|}{794} & \multicolumn{1}{c|}{915} & \multicolumn{1}{c|}{763} & \multicolumn{1}{c|}{882} & \multicolumn{1}{c|}{1.46} & \multicolumn{1}{c|}{1.45} & \multicolumn{1}{c|}{1.5} & \multicolumn{1}{c|}{1.51} & \multicolumn{1}{c|}{1.57} & 1.56 \\ \hline
% 10 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.37} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{826} & \multicolumn{1}{c|}{953} & \multicolumn{1}{c|}{799} & \multicolumn{1}{c|}{922} & \multicolumn{1}{c|}{772} & \multicolumn{1}{c|}{891} & \multicolumn{1}{c|}{1.45} & \multicolumn{1}{c|}{1.44} & \multicolumn{1}{c|}{1.49} & \multicolumn{1}{c|}{1.49} & \multicolumn{1}{c|}{1.55} & 1.54 \\ \hline


% \end{tabular}

%      \begin{tablenotes} \footnotesize
%        \item [a] Baseline receiver system, ORBGRAND decoding followed by AES decryption
%        \item [b] Proposed receiver system, joint decoding and decryption
%      \end{tablenotes}
%   \end{threeparttable}
%      }
% \end{table*}
    


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{2}
\begin{threeparttable}
\centering    
\caption{\centering Performance comparison in different receiver architectures}
\label{tab:hardware_results}
\begin{tabular}{|
>{\columncolor[HTML]{ffffff}}c ||
>{\columncolor[HTML]{DAE8FC}}c 
>{\columncolor[HTML]{E2F0D9}}c 
>{\columncolor[HTML]{FBE5D6}}c 
>{\columncolor[HTML]{E2F0D9}}c 
>{\columncolor[HTML]{FBE5D6}}c 
>{\columncolor[HTML]{DAE8FC}}c 
>{\columncolor[HTML]{E2F0D9}}c 
>{\columncolor[HTML]{FBE5D6}}c 
>{\columncolor[HTML]{E2F0D9}}c 
>{\columncolor[HTML]{FBE5D6}}c 
>{\columncolor[HTML]{DAE8FC}}c 
>{\columncolor[HTML]{E2F0D9}}c 
>{\columncolor[HTML]{FBE5D6}}c 
>{\columncolor[HTML]{DAE8FC}}c 
>{\columncolor[HTML]{E2F0D9}}c 
>{\columncolor[HTML]{FBE5D6}}c 
>{\columncolor[HTML]{DAE8FC}}c 
>{\columncolor[HTML]{E2F0D9}}c 
>{\columncolor[HTML]{FBE5D6}}c 
>{\columncolor[HTML]{DAE8FC}}c 
>{\columncolor[HTML]{E2F0D9}}c 
>{\columncolor[HTML]{FBE5D6}}c |}
\hline
 & \multicolumn{22}{c|}{\textbf{Number of Padding Bits (n-k)}} \\ \cline{2-23} 
 & \multicolumn{1}{c|}{*} & \multicolumn{2}{c|}{\textbf{8-bit}} & \multicolumn{2}{c||}{\textbf{12-bit}} & \multicolumn{1}{c|}{*} & \multicolumn{2}{c|}{\textbf{8-bit}} & \multicolumn{2}{c||}{\textbf{12-bit}} & \multicolumn{3}{c|}{\textbf{8-bit}} & \multicolumn{3}{c||}{\textbf{12-bit}} & \multicolumn{3}{c|}{\textbf{8-bit}} & \multicolumn{3}{c|}{\textbf{12-bit}} \\ \cline{2-23} 
 & \multicolumn{1}{c|}{\cellcolor[HTML]{DEEBF7}{\color[HTML]{3531FF} \textbf{B}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}{\color[HTML]{009901} \textbf{S}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}{\color[HTML]{CB0000} \textbf{P}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}{\color[HTML]{009901} \textbf{S}}} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}{\color[HTML]{CB0000} \textbf{P}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}{\color[HTML]{3531FF} \textbf{B}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}{\color[HTML]{009901} \textbf{S}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}{\color[HTML]{CB0000} \textbf{P}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}{\color[HTML]{009901} \textbf{S}}} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}{\color[HTML]{CB0000} \textbf{P}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}{\color[HTML]{3531FF} \textbf{B}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}{\color[HTML]{009901} \textbf{S}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}{\color[HTML]{CB0000} \textbf{P}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{B}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}{\color[HTML]{009901} \textbf{S}}} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}{\color[HTML]{CB0000} \textbf{P}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}{\color[HTML]{3531FF} \textbf{B}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}{\color[HTML]{009901} \textbf{S}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}{\color[HTML]{CB0000} \textbf{P}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}{\color[HTML]{3531FF} \textbf{B}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}{\color[HTML]{009901} \textbf{S}}} & {\color[HTML]{CB0000} \textbf{P}} \\ \cline{2-23} 
\multirow{-4}{*}{\textbf{Eb/N0}} & \multicolumn{5}{c||}{\textbf{Power (mW)}} & \multicolumn{5}{c||}{\textbf{Latency (ns)}} & \multicolumn{6}{c||}{\textbf{Goodput (Mbps)}} & \multicolumn{6}{c|}{\textbf{Energy/bit (pJ/bit)}} \\ \hline \hline
5 & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}\notableentry } & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1.4} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}0.4} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}1.35} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}471} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1683} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}226} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}508} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}129} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}64} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}22} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}17} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}5.36} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}21.9} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}18.3} & 78.8 \\ \cline{1-1} \cline{3-6} \cline{8-11} \cline{13-14} \cline{16-17} \cline{19-20} \cline{22-23} 
6 & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.09} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1.4} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.01} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}1.4} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}194} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}429} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}179} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}248} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}443} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}321} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}203} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}176} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}2.47} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}4.37} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}5.00} & 7.93 \\ \cline{1-1} \cline{3-6} \cline{8-11} \cline{13-14} \cline{16-17} \cline{19-20} \cline{22-23} 
7 & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.19} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1.39} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.19} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}1.4} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}159} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}160} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}157} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}157} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}690} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}726} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}596} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}627} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.72} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1.92} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.99} & 2.23 \\ \cline{1-1} \cline{3-6} \cline{8-11} \cline{13-14} \cline{16-17} \cline{19-20} \cline{22-23} 
8 & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.19} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1.38} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.21} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}1.38} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}152} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}136} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}152} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}136} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}771} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}878} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}728} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}832} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.54} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1.57} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.65} & 1.66 \\ \cline{1-1} \cline{3-6} \cline{8-11} \cline{13-14} \cline{16-17} \cline{19-20} \cline{22-23} 
9 & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.19} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1.38} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.2} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}1.38} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}150} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}131} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}150} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}131} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}794} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}915} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}763} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}882} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1.51} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.57} & 1.56 \\ \cline{1-1} \cline{3-6} \cline{8-11} \cline{13-14} \cline{16-17} \cline{19-20} \cline{22-23} 
10 & \multicolumn{1}{c|}{\multirow{-6}{*}{\cellcolor[HTML]{DAE8FC}1.21}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.19} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1.38} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.2} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}1.38} & \multicolumn{1}{c|}{\multirow{-6}{*}{\cellcolor[HTML]{DAE8FC}130}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}150} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}130} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}150} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}130} & \multicolumn{1}{c|}{\multirow{-6}{*}{\cellcolor[HTML]{DAE8FC}923}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}799} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}923} & \multicolumn{1}{c|}{\multirow{-6}{*}{\cellcolor[HTML]{DAE8FC}892}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}772} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}892} & \multicolumn{1}{c|}{\multirow{-6}{*}{\cellcolor[HTML]{DAE8FC}1.30}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.49} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1.49} & \multicolumn{1}{c|}{\multirow{-6}{*}{\cellcolor[HTML]{DAE8FC}1.34}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.55} & 1.54 \\ \hline
\end{tabular}
     \begin{tablenotes} \footnotesize
       \item {\color[HTML]{3531FF}B: Baseline receiver system, AES decryption only}
       \item {\color[HTML]{009901}S: Separate receiver system, ORBGRAND decoding followed by AES decryption}
       \item {\color[HTML]{CB0000}P: Proposed receiver system, joint ORBGRAND decoding and AES decryption}
     \end{tablenotes}
  \end{threeparttable}}
\end{table*}







==> tables/table_with_all_no_op.tex <==

    
\newlength{\Oldarrayrulewidth}
\newcommand{\Cline}[2]{%
  \noalign{\global\setlength{\Oldarrayrulewidth}{\arrayrulewidth}}%
  \noalign{\global\setlength{\arrayrulewidth}{#1}}\cline{#2}%
  \noalign{\global\setlength{\arrayrulewidth}{\Oldarrayrulewidth}}}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{2}
\begin{threeparttable}
\centering    
\caption{\centering Performance comparison in different receiver architectures \\ (Goodput is valid for BER $< 10^{-4}$)}
\label{tab:hardware_results}
\begin{tabular}{|
c ||
>{\columncolor[HTML]{DAE8FC}}c 
>{\columncolor[HTML]{E2F0D9}}c 
>{\columncolor[HTML]{FBE5D6}}c 
>{\columncolor[HTML]{E2F0D9}}c 
>{\columncolor[HTML]{FBE5D6}}c 
>{\columncolor[HTML]{DAE8FC}}c 
>{\columncolor[HTML]{E2F0D9}}c 
>{\columncolor[HTML]{FBE5D6}}c 
>{\columncolor[HTML]{E2F0D9}}c 
>{\columncolor[HTML]{FBE5D6}}c 
>{\columncolor[HTML]{DAE8FC}}c 
>{\columncolor[HTML]{E2F0D9}}c 
>{\columncolor[HTML]{FBE5D6}}c 
>{\columncolor[HTML]{DAE8FC}}c 
>{\columncolor[HTML]{E2F0D9}}c 
>{\columncolor[HTML]{FBE5D6}}c 
>{\columncolor[HTML]{DAE8FC}}c 
>{\columncolor[HTML]{E2F0D9}}c 
>{\columncolor[HTML]{FBE5D6}}c 
>{\columncolor[HTML]{DAE8FC}}c 
>{\columncolor[HTML]{E2F0D9}}c 
>{\columncolor[HTML]{FBE5D6}}c |l}
\cline{1-23}
 & \multicolumn{22}{c|}{\textbf{Number of Padding Bits (n-k)}} \\ \cline{2-23} 
 & \multicolumn{1}{c|}{*} & \multicolumn{2}{c|}{\textbf{8-bit}} & \multicolumn{2}{c||}{\textbf{12-bit}} & \multicolumn{1}{c|}{*} & \multicolumn{2}{c|}{\textbf{8-bit}} & \multicolumn{2}{c||}{\textbf{12-bit}} & \multicolumn{3}{c|}{\textbf{8-bit}} & \multicolumn{3}{c||}{\textbf{12-bit}} & \multicolumn{3}{c|}{\textbf{8-bit}} & \multicolumn{3}{c|}{\textbf{12-bit}} \\ \cline{2-23} 
 & \multicolumn{1}{c|}{\cellcolor[HTML]{DEEBF7}{\color[HTML]{3531FF} \textbf{B}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}{\color[HTML]{009901} \textbf{S}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}{\color[HTML]{CB0000} \textbf{P}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}{\color[HTML]{009901} \textbf{S}}} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}{\color[HTML]{CB0000} \textbf{P}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}{\color[HTML]{3531FF} \textbf{B}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}{\color[HTML]{009901} \textbf{S}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}{\color[HTML]{CB0000} \textbf{P}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}{\color[HTML]{009901} \textbf{S}}} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}{\color[HTML]{CB0000} \textbf{P}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}{\color[HTML]{3531FF} \textbf{B}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}{\color[HTML]{009901} \textbf{S}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}{\color[HTML]{CB0000} \textbf{P}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{B}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}{\color[HTML]{009901} \textbf{S}}} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}{\color[HTML]{CB0000} \textbf{P}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}{\color[HTML]{3531FF} \textbf{B}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}{\color[HTML]{009901} \textbf{S}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}{\color[HTML]{CB0000} \textbf{P}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}{\color[HTML]{3531FF} \textbf{B}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}{\color[HTML]{009901} \textbf{S}}} & {\color[HTML]{CB0000} \textbf{P}} \\ \cline{2-23} 
\multirow{-4}{*}{\textbf{Eb/N0}} & \multicolumn{5}{c||}{\textbf{Power (mW)}} & \multicolumn{5}{c||}{\textbf{Latency (ns)}} & \multicolumn{6}{c||}{\textbf{Goodput (Mbps)}} & \multicolumn{6}{c|}{\textbf{Energy/bit (pJ/bit)}} \\ \cline{1-23} \cline{1-23}
5.5 & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}\textbf{N/A} } & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}\textbf{N/A}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}0.4} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}1.35} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}\textbf{N/A}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}\textbf{N/A}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}226} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}508} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}\textbf{N/A}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}\textbf{N/A}} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}22} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}17} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}\textbf{N/A}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}\textbf{N/A}} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}18.3} & 78.8 \\ \cline{1-1} \cline{3-6} \cline{8-11} \cline{13-14} \cline{16-17} \cline{19-20} \cline{22-23} 
6 & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.09} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1.4} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.01} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}1.4} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}194} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}429} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}179} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}248} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}443} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}321} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}203} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}176} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}2.47} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}4.37} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}5.00} & 7.93 \\ \cline{1-1} \cline{3-6} \cline{8-11} \cline{13-14} \cline{16-17} \cline{19-20} \cline{22-23} 
7 & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.19} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1.39} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.19} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}1.4} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}159} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}160} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}157} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}157} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}690} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}726} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}596} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}627} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.72} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1.92} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.99} & 2.23 \\ \cline{1-1} \cline{3-6} \cline{8-11} \cline{13-14} \cline{16-17} \cline{19-20} \cline{22-23} 
8 & \multicolumn{1}{c|}{\multirow{-4}{*}{\cellcolor[HTML]{DAE8FC}\textbf{N/A}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.19} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1.38} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.21} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}1.38} & \multicolumn{1}{c|}{\multirow{-4}{*}{\cellcolor[HTML]{DAE8FC}\textbf{N/A}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}152} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}136} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}152} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}136} & \multicolumn{1}{c|}{\multirow{-4}{*}{\cellcolor[HTML]{DAE8FC}\textbf{N/A}}}& \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}771} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}878} & \multicolumn{1}{c|}{\multirow{-4}{*}{\cellcolor[HTML]{DAE8FC}\textbf{N/A}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}728} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}832} & \multicolumn{1}{c|}{\multirow{-4}{*}{\cellcolor[HTML]{DAE8FC}\textbf{N/A}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.54} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1.57} & \multicolumn{1}{c|}{\multirow{-4}{*}{\cellcolor[HTML]{DAE8FC}\textbf{N/A}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.65} & 1.66 & \multicolumn{1}{c}{\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}dBs for Nothing\\ FEC for Free\end{tabular}}} \\ \cline{1-23} \cline{1-23} 
9 & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.19} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1.38} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.2} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}1.38} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}150} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}131} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}150} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}131} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}794} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}915} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}763} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}882} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1.51} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.57} & 1.56 \\ \cline{1-1} \cline{3-6} \cline{8-11} \cline{13-14} \cline{16-17} \cline{19-20} \cline{22-23}
10 & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{DAE8FC}1.21}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.19} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1.38} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.2} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}1.38} & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{DAE8FC}130}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}150} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}130} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}150} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}130} & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{DAE8FC}923}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}799} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}923} & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{DAE8FC}892}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}772} & \multicolumn{1}{c||}{\cellcolor[HTML]{FBE5D6}892} & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{DAE8FC}1.30}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.49} & \multicolumn{1}{c|}{\cellcolor[HTML]{FBE5D6}1.49} & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{DAE8FC}1.34}} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F0D9}1.55} & 1.54 \\ \cline{1-23}
\end{tabular}
     \begin{tablenotes} \footnotesize
       \item {\color[HTML]{3531FF}B: Baseline receiver system, AES decryption only}
       \item {\color[HTML]{009901}S: Separate receiver system, ORBGRAND decoding followed by AES decryption}
       \item {\\ \color[HTML]{CB0000} P: Proposed receiver system, joint ORBGRAND decoding and AES decryption}
       \item {\textbf{N/A}: Unavailable due to high BER in the initial transmission}
     \end{tablenotes}
  \end{threeparttable}}
\end{table*}







==> tables/table_with_latency.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}

% \begin{table*}[]
% \resizebox{\textwidth}{!}{%
% \renewcommand{\arraystretch}{2}
% \begin{threeparttable}
% \centering    
% \caption{\centering Performance comparison in different with different numbers of splits}
% \label{tab:hardware_results}

% \begin{tabular}{|c|cccccccccccccccccc|}
% \hline
% \multirow{4}{*}{\textbf{EbN0}} & \multicolumn{6}{c|}{\textbf{Power   (mW)}} & \multicolumn{6}{c|}{\textbf{Goodput   (Mbps)}} & \multicolumn{6}{c|}{\textbf{Energy/bit   (pJ/bit)}} \\ \cline{2-19} 
%  & \multicolumn{18}{c|}{\textbf{Code   rate (R)}} \\ \cline{2-19} 
%  & \multicolumn{2}{c|}{\textbf{4-bit}} & \multicolumn{2}{c|}{\textbf{8-bit}} & \multicolumn{2}{c|}{\textbf{12-bit}} & \multicolumn{2}{c|}{\textbf{4-bit}} & \multicolumn{2}{c|}{\textbf{8-bit}} & \multicolumn{2}{c|}{\textbf{12-bit}} & \multicolumn{2}{c|}{\textbf{4-bit}} & \multicolumn{2}{c|}{\textbf{8-bit}} & \multicolumn{2}{c|}{\textbf{12-bit}} \\ \cline{2-19} 
%  & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \textbf{P} \\ \hline\hline
% 5 & \multicolumn{1}{c|}{1.05} & \multicolumn{1}{c|}{1.46} & \multicolumn{1}{c|}{0.69} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{0.4} & \multicolumn{1}{c|}{1.35} & \multicolumn{1}{c|}{469} & \multicolumn{1}{c|}{238} & \multicolumn{1}{c|}{129} & \multicolumn{1}{c|}{64} & \multicolumn{1}{c|}{22} & \multicolumn{1}{c|}{17} & \multicolumn{1}{c|}{2.24} & \multicolumn{1}{c|}{6.14} & \multicolumn{1}{c|}{5.36} & \multicolumn{1}{c|}{21.9} & \multicolumn{1}{c|}{18.3} & 78.8 \\ \hline
% 6 & \multicolumn{1}{c|}{1.15} & \multicolumn{1}{c|}{1.42} & \multicolumn{1}{c|}{1.09} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{1.01} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{644} & \multicolumn{1}{c|}{529} & \multicolumn{1}{c|}{443} & \multicolumn{1}{c|}{321} & \multicolumn{1}{c|}{203} & \multicolumn{1}{c|}{176} & \multicolumn{1}{c|}{1.79} & \multicolumn{1}{c|}{2.69} & \multicolumn{1}{c|}{2.47} & \multicolumn{1}{c|}{4.37} & \multicolumn{1}{c|}{5.00} & 7.93 \\ \hline
% 7 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.39} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.39} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{758} & \multicolumn{1}{c|}{812} & \multicolumn{1}{c|}{690} & \multicolumn{1}{c|}{726} & \multicolumn{1}{c|}{596} & \multicolumn{1}{c|}{627} & \multicolumn{1}{c|}{1.58} & \multicolumn{1}{c|}{1.71} & \multicolumn{1}{c|}{1.72} & \multicolumn{1}{c|}{1.92} & \multicolumn{1}{c|}{1.99} & 2.23 \\ \hline
% 8 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{808} & \multicolumn{1}{c|}{919} & \multicolumn{1}{c|}{771} & \multicolumn{1}{c|}{878} & \multicolumn{1}{c|}{728} & \multicolumn{1}{c|}{832} & \multicolumn{1}{c|}{1.48} & \multicolumn{1}{c|}{1.5} & \multicolumn{1}{c|}{1.54} & \multicolumn{1}{c|}{1.57} & \multicolumn{1}{c|}{1.65} & 1.66 \\ \hline
% 9 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.37} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{823} & \multicolumn{1}{c|}{947} & \multicolumn{1}{c|}{794} & \multicolumn{1}{c|}{915} & \multicolumn{1}{c|}{763} & \multicolumn{1}{c|}{882} & \multicolumn{1}{c|}{1.46} & \multicolumn{1}{c|}{1.45} & \multicolumn{1}{c|}{1.5} & \multicolumn{1}{c|}{1.51} & \multicolumn{1}{c|}{1.57} & 1.56 \\ \hline
% 10 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.37} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{826} & \multicolumn{1}{c|}{953} & \multicolumn{1}{c|}{799} & \multicolumn{1}{c|}{922} & \multicolumn{1}{c|}{772} & \multicolumn{1}{c|}{891} & \multicolumn{1}{c|}{1.45} & \multicolumn{1}{c|}{1.44} & \multicolumn{1}{c|}{1.49} & \multicolumn{1}{c|}{1.49} & \multicolumn{1}{c|}{1.55} & 1.54 \\ \hline


% \end{tabular}

%      \begin{tablenotes} \footnotesize
%        \item [a] Baseline receiver system, ORBGRAND decoding followed by AES decryption
%        \item [b] Proposed receiver system, joint decoding and decryption
%      \end{tablenotes}
%   \end{threeparttable}
%      }
% \end{table*}
    
    


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{2}
\begin{threeparttable}
\centering    
\caption{\centering Performance comparison in different receiver architectures}
\label{tab:hardware_results}
\begin{tabular}{|c||cccccccccccccccccccccccc|}
\hline
\multirow{4}{*}{\textbf{EbN0}} & \multicolumn{24}{c|}{\textbf{Number of Redundancy Bits (n-k)}} \\ \cline{2-25} 
 & \multicolumn{2}{c|}{\textbf{4-bit}} & \multicolumn{2}{c|}{\textbf{8-bit}} & \multicolumn{2}{c||}{\textbf{12-bit}} & \multicolumn{2}{c|}{\textbf{4-bit}} & \multicolumn{2}{c|}{\textbf{8-bit}} & \multicolumn{2}{c||}{\textbf{12-bit}} & \multicolumn{2}{c|}{\textbf{4-bit}} & \multicolumn{2}{c|}{\textbf{8-bit}} & \multicolumn{2}{c||}{\textbf{12-bit}} & \multicolumn{2}{c|}{\textbf{4-bit}} & \multicolumn{2}{c|}{\textbf{8-bit}} & \multicolumn{2}{c|}{\textbf{12-bit}} \\ \cline{2-25} 
 & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c||}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c||}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c||}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{B}} & \textbf{P} \\ \cline{2-25} 
 & \multicolumn{6}{c||}{Power (mW)} & \multicolumn{6}{c||}{Latency (ns)} & \multicolumn{6}{c||}{Goodput (Mbps)} & \multicolumn{6}{c|}{Energy/bit (pJ/bit)} \\ \hline \hline
5 & \multicolumn{1}{c|}{1.05} & \multicolumn{1}{c|}{1.46} & \multicolumn{1}{c|}{0.69} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{0.4} & \multicolumn{1}{c||}{1.35} & \multicolumn{1}{c|}{1482} & \multicolumn{1}{c|}{7995} & \multicolumn{1}{c|}{471} & \multicolumn{1}{c|}{1683} & \multicolumn{1}{c|}{226} & \multicolumn{1}{c||}{508} & \multicolumn{1}{c|}{469} & \multicolumn{1}{c|}{238} & \multicolumn{1}{c|}{129} & \multicolumn{1}{c|}{64} & \multicolumn{1}{c|}{22} & \multicolumn{1}{c||}{17} & \multicolumn{1}{c|}{2.24} & \multicolumn{1}{c|}{6.14} & \multicolumn{1}{c|}{5.36} & \multicolumn{1}{c|}{21.9} & \multicolumn{1}{c|}{18.3} & 78.8 \\ \hline
6 & \multicolumn{1}{c|}{1.15} & \multicolumn{1}{c|}{1.42} & \multicolumn{1}{c|}{1.09} & \multicolumn{1}{c|}{1.4} & \multicolumn{1}{c|}{1.01} & \multicolumn{1}{c||}{1.4} & \multicolumn{1}{c|}{224} & \multicolumn{1}{c|}{593} & \multicolumn{1}{c|}{194} & \multicolumn{1}{c|}{429} & \multicolumn{1}{c|}{179} & \multicolumn{1}{c||}{248} & \multicolumn{1}{c|}{644} & \multicolumn{1}{c|}{529} & \multicolumn{1}{c|}{443} & \multicolumn{1}{c|}{321} & \multicolumn{1}{c|}{203} & \multicolumn{1}{c||}{176} & \multicolumn{1}{c|}{1.79} & \multicolumn{1}{c|}{2.69} & \multicolumn{1}{c|}{2.47} & \multicolumn{1}{c|}{4.37} & \multicolumn{1}{c|}{5.00} & 7.93 \\ \hline
7 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.39} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.39} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c||}{1.4} & \multicolumn{1}{c|}{162} & \multicolumn{1}{c|}{174} & \multicolumn{1}{c|}{159} & \multicolumn{1}{c|}{160} & \multicolumn{1}{c|}{157} & \multicolumn{1}{c||}{157} & \multicolumn{1}{c|}{758} & \multicolumn{1}{c|}{812} & \multicolumn{1}{c|}{690} & \multicolumn{1}{c|}{726} & \multicolumn{1}{c|}{596} & \multicolumn{1}{c||}{627} & \multicolumn{1}{c|}{1.58} & \multicolumn{1}{c|}{1.71} & \multicolumn{1}{c|}{1.72} & \multicolumn{1}{c|}{1.92} & \multicolumn{1}{c|}{1.99} & 2.23 \\ \hline
8 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c||}{1.38} & \multicolumn{1}{c|}{153} & \multicolumn{1}{c|}{139} & \multicolumn{1}{c|}{152} & \multicolumn{1}{c|}{136} & \multicolumn{1}{c|}{152} & \multicolumn{1}{c||}{136} & \multicolumn{1}{c|}{808} & \multicolumn{1}{c|}{919} & \multicolumn{1}{c|}{771} & \multicolumn{1}{c|}{878} & \multicolumn{1}{c|}{728} & \multicolumn{1}{c||}{832} & \multicolumn{1}{c|}{1.48} & \multicolumn{1}{c|}{1.5} & \multicolumn{1}{c|}{1.54} & \multicolumn{1}{c|}{1.57} & \multicolumn{1}{c|}{1.65} & 1.66 \\ \hline
9 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.37} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c||}{1.38} & \multicolumn{1}{c|}{151} & \multicolumn{1}{c|}{131} & \multicolumn{1}{c|}{150} & \multicolumn{1}{c|}{131} & \multicolumn{1}{c|}{150} & \multicolumn{1}{c||}{131} & \multicolumn{1}{c|}{823} & \multicolumn{1}{c|}{947} & \multicolumn{1}{c|}{794} & \multicolumn{1}{c|}{915} & \multicolumn{1}{c|}{763} & \multicolumn{1}{c||}{882} & \multicolumn{1}{c|}{1.46} & \multicolumn{1}{c|}{1.45} & \multicolumn{1}{c|}{1.5} & \multicolumn{1}{c|}{1.51} & \multicolumn{1}{c|}{1.57} & 1.56 \\ \hline
10 & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{1.37} & \multicolumn{1}{c|}{1.19} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c||}{1.38} & \multicolumn{1}{c|}{150} & \multicolumn{1}{c|}{130} & \multicolumn{1}{c|}{150} & \multicolumn{1}{c|}{130} & \multicolumn{1}{c|}{150} & \multicolumn{1}{c||}{130} & \multicolumn{1}{c|}{826} & \multicolumn{1}{c|}{953} & \multicolumn{1}{c|}{799} & \multicolumn{1}{c|}{922} & \multicolumn{1}{c|}{772} & \multicolumn{1}{c||}{891} & \multicolumn{1}{c|}{1.45} & \multicolumn{1}{c|}{1.44} & \multicolumn{1}{c|}{1.49} & \multicolumn{1}{c|}{1.49} & \multicolumn{1}{c|}{1.55} & 1.54 \\ \hline



\end{tabular}

     \begin{tablenotes} \footnotesize
       \item B: Baseline receiver system, ORBGRAND decoding followed by AES decryption
       \item P: Proposed receiver system, joint ORBGRAND decoding and AES decryption
     \end{tablenotes}
  \end{threeparttable}
     }
\end{table*}






